Transform coder identification based on quantization footprints and lattice theory

Transform coding is routinely used for lossy compression of discrete sources with memory. The input signal is divided into N-dimensional vectors, which are transformed by means of a linear mapping. Then, transform coefficients are quantized and entropy coded. In this paper we consider the problem of identifying the transform matrix as well as the quantization step sizes. We study the challenging case in which the only available information is a set of P transform decoded vectors. We formulate the problem in terms of finding the lattice with the largest determinant that contains all observed vectors. We propose an algorithm that is able to find the optimal solution and we formally study its convergence properties. Our analysis shows that it is possible to identify successfully both the transform and the quantization step sizes when P >= N + d where d is a small integer, and the probability of failure decreases exponentially to zero as P - N increases.

==> 1_Introduction.tex <==
\section{Introduction}
Transform coding has emerged over the years as the dominating compression strategy. Transform coding is adopted in virtually all multimedia compression standards including image compression standards such as JPEG~\cite{Wallace1991} and JPEG 2000~\cite{TaubmanM:2002,Lee2005} and video compression standards such as, for example, H.264/AVC~\cite{Sullivan2005} and HEVC~\cite{WikenHMSW:2011}. This is due to the fact that transform coders are very effective and yet computationally inexpensive since the encoding operation is divided into three relatively simple steps: the computation of a linear transformation of the data, scalar quantization of each coefficient, and entropy coding.

Transform coding has been widely studied in the last decades and many important results and optimality conditions have been derived. For example, it is well known that, for Gaussian sources, the Karhunen-Lo\`eve Transform (KLT) is the optimal transform~\cite{HuangS:63}\cite{Goyal:SPM2001}. Moreover, the analysis of popular transform coders used in image compression has also led to new insights and new interesting connections between compression and non-linear approximation theory~\cite{Vetterli:01}. In particular, this analysis has also clarified why the wavelet transform is the best transform for compressing piecewise regular functions~\cite{CohenDGO:01}\cite{Mallat:98}. Further insights on the interplay between linear transform, quantization and entropy coding can be found in~\cite{Goyal:00} for the case of integer-to-integer transforms. 

Due to its centrality to any type of multimedia data, transform coding theory is now extensively used in a new range of applications that rely on the possibility of reverse-engineering complex chains of operators starting from the available output signals. Indeed, the lifespan of a multimedia signal is virtually unbounded. This is due to the ability of creating copies and the availability of inexpensive storage options. However, signals seldom remain identical to their original version. As they pass through processing chains, some operators, including transform coding, are bound to leave subtle characteristic footprints on the signals, which can be identified in order to uncover their processing history. This insight might be extremely useful in a wide range of scenarios in the field of multimedia signal processing at large including, e.g.,: i) forensics, in order to address tasks such as source device identification~\cite{LukasFG:TIFS2006} or tampering detection~\cite{ChenFGL:TIFS2008}\cite{BianchiP:TIFS2012}; ii) quality assessment, to enable no-reference methods that rely solely on the received signals~\cite{ValenziseMTT:TCSVT2012}\cite{NaccariTT:TMM2009}; iii) digital restoration, which requires prior knowledge about the operations that affected a digital signal~\cite{BanhamK:SPM1997}. 

In this context, several works have exploited the footprints left by transform coding. In~\cite{FanQ:TIP2003}, a method was proposed to infer the implementation-dependent quantization matrix template used in a JPEG-compressed image. Double JPEG compression introduces characteristic peaks in the histogram of DCT coefficients, which can be detected and used, e.g, for tampering localization~\cite{LukasF:DFRW03}\cite{BianchiP:TIFS2012}. More recently, similar techniques were applied to video signals for the cases of MPEG-2~\cite{ChenCB:ICIP1998}\cite{LiF:PCS2009}, MPEG-4~\cite{LuoWH:SPIE2008}\cite{WangF:ACMMMSec2009} and H.264/AVC~\cite{TagliasacchiT:2010}. 

All the aforementioned works require prior knowledge of the type of standard being considered. This implies that the specific transform in use is assumed to be known, whereas the quantization step sizes need to be estimated. 
In practice, it might be useful to be able to infer which transform was used in order to understand, for example, whether an image was compressed using 
the  DCT-based JPEG or the wavelet-based JPEG 2000 and, in the latter case, which wavelet transform was used. Similarly, it would be good to be able to 
infer if a video sequence was compressed using MPEG-2, MPEG-4 or H.264/AVC. Some efforts in this direction can be found in~\cite{BestaginiAMTT:2012}.
 
Most of the above methods focus only on a specific type of multimedia signal (e.g., only images or only videos) and are to some extent heuristic. It is therefore natural to try and develop a universal theory of transform coder identification that is independent of the specific application at hand. To this end, in this paper we consider a general model of transform coding that can be tailored to describe a large variety of practical implementations that are found in lossy coding systems, including those adopted in multimedia communication. Specifically, a 1-dimensional input signal is encoded by partitioning it into non-overlapping $N$-dimensional vectors, which are then transformed by means of a linear mapping. Then, transform coefficients are quantized and entropy coded. At the decoder, quantization symbols are entropy decoded and mapped to reconstruction levels. Then, the inverse transform is applied to obtain an approximation of the signal in its original domain.

Given the output produced by a specific transform coding chain, we investigate the problem of identifying its parameters. To this end, we assume both the size and the alignment of the transform to be known, as they can be estimated with methods available in the literature~\cite{LiF:PCS2009}\cite{FanQ:TIP2003}. We propose an algorithm that receives as input a set of $\Points$ transform decoded vectors embedded in a $\Dim$-dimensional vector space and produces as output an estimation of the transform adopted, as well as the quantization step sizes, whenever these can be unambiguously determined. We leverage the intrinsic discrete nature of the problem, by observing the fact that these vectors are bound to belong to a $\Dim$-dimensional lattice. Hence, the problem is formulated in terms of finding a lattice 
that contains all observed vectors. We propose an algorithm that is able to solve the problem and we formally study its convergence properties. Our analysis shows that it is possible to successfully identify both the transform and the quantization step sizes with high probability when $\Points > \Dim$. In the experiments we found that an excess of approximately 6-7 observed vectors beyond the dimension $\Dim$ of the space is generally 
sufficient to ensure successful convergence. In addition, the complexity of the algorithm is shown to grow linearly with $\Dim$.

It is important to mention that the method used to solve the problem addressed in this paper is related to Euclid's algorithm, which is used to find the greatest common divisor (GCD) in a set of integers. 
Indeed, when $\Dim = 1$ and $\Points = 2$, the proposed method coincides with Euclid's algorithm. However, in this case the problem reduces to estimating the quantization step size, as the transform is trivially defined. 

Note that,
lattice theory has been widely used for source and channel coding (e.g.,~\cite{GrayN:98, ZamirSE:02,WubberSJM:SMP2011}). However,
to the best of the authors' knowledge, this theory has not been 
employed to address the
 problem of identifying a linear mapping using the footprint left by quantization. Only~\cite{NeelamaniQZB:2006} uses similar principles but their goal is to investigate the color compression history, i.e., the colorspace used in JPEG compression. Therefore, the solution proposed is tailored to work in a 3-dimensional vector space, thus avoiding the challenges that arise in higher dimensional spaces.  


Also, it is important not to confuse the problem addressed in this paper with the classical problem of lattice reduction~\cite{WubberSJM:SMP2011}. In the latter case, given a basis for a lattice, one seeks an equivalent basis matrix with favorable properties. Usually, such a basis consists of vectors that are short and with improved orthogonality. There are several definitions of lattice reduction with corresponding reduction criteria, each meeting a different tradeoff between quality of the reduced basis and the computational effort required for finding it. The most popular one is the Lenstra-Lenstra-Lovasz (LLL) reduction~\cite{LenstraLL:MA1982}, which can be interpreted as an extension of the Gauss reduction to lattices of rank greater than 2.



The rest of this paper is organized as follows. Section~\ref{sec:setup} introduces the necessary notation and formulates the transform identification problem and Section~\ref{sec:lattices} provides the background on lattice theory. The proposed method is described in Section~\ref{sec:transformidentification}. Then, a theoretical analysis of the convergence properties is presented in Section~\ref{sec:analysis}. The performance of the transform identification algorithm is evaluated empirically in Section~\ref{sec:experiments}. Finally, Section~\ref{sec:conclusions} concludes the paper, indicating the open issues and stimulating further investigations. 
 


==> 8_Conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}
In this paper we proposed a method which is able to identify the parameters of a transform coder from a set of $\Points$ transform decoded vectors embedded in a $\Dim$-dimensional space. We proved that it is possible to successfully identify the transform and the quantization step sizes when $\Points > \Dim$ and this despite of the huge number of potential quantization bins, which grows exponentially with $\Dim$ for a target bitrate. In addition, we proved that the probability of failure decreases exponentially to zero when $\Points - \Dim$ increases. In our experiments we found that an excess of approximately 6-7 observed vectors beyond the dimension $\Dim$ of the space is generally sufficient to ensure successful convergence. 

In this paper, we focused on a noiseless scenario, in which we observe directly the output of the decoder. In some cases, though, signals are processed in complex chains, in which multiple transform coders are cascaded, thus introducing noise in the observed vectors. 
Consequently, the observed vectors do not lie exactly on lattice points.
Extending the proposed method to this new scenario represents an interesting 
research avenue to be investigated.

\balance

